Guiding AMR Parsing with Reverse Graph Linearization

Abstract Meaning Representation (AMR) parsing aims to extract an abstract semantic graph from a given sentence. The sequence-to-sequence approaches, which linearize the semantic graph into a sequence of nodes and edges and generate the linearized graph directly, have achieved good performance. However, we observed that these approaches suffer from structure loss accumulation during the decoding process, leading to a much lower F1-score for nodes and edges decoded later compared to those decoded earlier. To address this issue, we propose a novel Reverse Graph Linearization (RGL) enhanced framework. RGL defines both default and reverse linearization orders of an AMR graph, where most structures at the back part of the default order appear at the front part of the reversed order and vice versa. RGL incorporates the reversed linearization to the original AMR parser through a two-pass self-distillation mechanism, which guides the model when generating the default linearizations. Our analysis shows that our proposed method significantly mitigates the problem of structure loss accumulation, outperforming the previously best AMR parsing model by 0.8 and 0.5 Smatch scores on the AMR 2.0 and AMR 3.0 dataset, respectively. The code are available at https://github.com/pkunlp-icler/AMR_reverse_graph_linearization.

==> src/dataset.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/amri.pdf}
    \caption{AMRization methods for SRL and DP}
    \label{fig:amrization}
\end{figure*}

\subsection{Auxiliary Task Selection}

we choose from a wide range of tasks including summarization\citep{Hermann2015TeachingMT,chen-etal-2021-dialogsum}, translation and parsing\citep{ptb3,Weischedel2017OntoNotesA} to evaluate the contribution of different auxiliary task for AMR parsing. We use gold annotation data in all tasks and maintain a close number (\textasciitilde40k) of examples for each task for fair comparison. Due to space limitation, we list the full dataset description in Appendix~\ref{app:dataset_des}. 

% \subsection{Summarization}

% \paragraph{\textsc{CNN/DM}\citep{Hermann2015TeachingMT}}The CNN / DailyMail Dataset is an English-language dataset containing news articles as written by journalists at CNN and the Daily Mail. The dataset is widely accepted as benchmark to test models' performance of summarizing . We select 40k training data for fair comparison. 
% \paragraph{\textsc{DialogSum}\citep{chen-etal-2021-dialogsum}}
% The Real-Life Scenario Dialogue Summarization (\textsc{DialogSum}), is a large-scale summarization dataset for dialogues. Unlike \textsc{CNN/DM} which focuses on monologue news summarization, \textsc{DialogSum} covers a wide range of daily-life topics in the form of spoken dialogue. We use all the training data (13k) to conduct the intermediate training.

% \subsection{Translation}

% \paragraph{\textsc{WMT14 EN-DE}} We select 40k training examples from WMT14 EN-DE training set to form EN-DE and DE-EN translation intermediate task.

% \subsection{Dependency Parsing}

% \paragraph{\textsc{Penn Treebank}\citep{ptb3}} The Penn Treebank (PTB) project selected 2,499 stories from a three year Wall Street Journal (WSJ) collection of 98,732 stories for syntactic annotation. We only utilize the dependency structure annotations to form our intermediate dependency parsing task. There are 39k sentences for dependency parsing. 

% \subsection{Semantic Role Labeling}
% \paragraph{\textsc{OntoNotes}\citep{Weischedel2017OntoNotesA}} The OntoNotes project is built on two resources, following the \textsc{Penn Treebank}\citep{ptb3} for syntax and the \textsc{Penn PropBank} for predicate-argument structure. We select 40k sentences with SRL annotations to form intermediate task.



% \include{AMRization/table/dataset}

==> src/task.tex <==
Following previous methods \cite{bevil-spring, xu-seqpretrain, ge-seq2seqamr}, we formulate AMR parsing as a sequence-to-sequence generation problem.
Formally, given a sentence $\mathbf{x} = (x_1, x_2, ..., x_N)$, the model needs to generate a linearized AMR graph $\mathbf{y}=(y_1, y_2, ..., y_M)$.
As shown in Figure \cite{xx},
following \cite{bevil-spring}, the AMR graph was linearized with Depth-First Search (DFS) traversal, and variables in AMR are set to a a series of special tokens \textit{<R0>, <R1>, ..., <Rk>}.



==> table/OOD.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \resizebox{0.35\textwidth}{!}{
\begin{tabular}{llccc}
        \toprule
          Model&BIO & TLP &News3 \\
        \midrule
         SPRING & 59.7 & 77.3 & 73.7\\
         SPRING + silver &59.5 & 77.5 &71.8 \\
         SPRING$^E$ & 60.5 & 77.9 &74.7 \\
         \textbf{Ours} &\textbf{61.2} & \textbf{78.9} & \textbf{75.4} \\
        
        \bottomrule
    \end{tabular}
    % }
    \caption{Analysis on OOD data. $^E$ denotes result given by the ensembling of models. Our model exploits SRL as the intermediate task.}

    \label{tab:ood}
\end{table}

==> table/amization_full.tex <==
 \begin{table*}[t]
    \centering
    \resizebox{0.9\textwidth}{!}{%
\begin{tabular}{llccccccccccc}
        \toprule
                ~& \multirow{2}{*}{Model} &\multirow{2}{*}{Extra Data} & \multirow{2}{*}{\textsc{smatch}} &
                \multirow{2}{*}{NoWSD} &
                \multirow{2}{*}{Wiki} &
                \multicolumn{3}{c}{Concept-related} & \multicolumn{3}{c}{Topology-related} \\
                \cmidrule(r){7-9} \cmidrule(r){10-12} 
        ~ & ~ & ~ & ~& ~ &~& Conc. & NER & Neg. & Unll. & Reen. & SRL \\
        \midrule
        

        \multirow{9}{*}{\rotatebox[origin=c]{90}{{AMR 2.0}}}     
         ~&SPRING (w/ silver) \citep{bevil-spring}    &200k     & 84.3 & 84.8& 83.1 & \textbf{90.8} & 90.5 & 73.6  &  86.7 &  72.4 & 80.5 \\
        

        ~& \textbf{Ours (w/ Semantic Role Labeling) } &40k &84.5 &84.9&84.0 &90.2 & 91.8&74.6&87.7 &74.2 &82.8 \\
        ~& - w/ Arg. Reduction(AR) &40k &84.8 &85.2&83.9 &90.4 &92.2 &74.2&88.1 & 74.5 &83.0  \\
        ~& - w/ Reen. Restoration(RR)  &40k &85.0 &85.4&83.5&90.6 & 92.1 &75.6&\textbf{88.2}&\textbf{75.5}&\textbf{83.7}\\
        ~& - w/ AR+RR  &40k    &\textbf{85.1}   &\textbf{85.6} &  83.6 &90.4  & 91.4  & \textbf{75.7}  & \textbf{88.2} & 75.0  &  83.5   \\
       
        ~& \textbf{Ours (w/ Dependency Parsing) } &40k  &84.4 &84.9& 82.9 &90.1&90.5 &73.5 &87.8 &74.3 &82.9 \\
        ~& - w/ Redundant Relation Removal (RRR) &40k & 84.5 & 	85.0	&83.5 	&90.2 	&91.2 	&74.3 	&88.0 &74.5 	&82.9  \\
        ~& - w/ Lemmatization (Lemma)  &40k & 84.7 	& 	85.2 &83.8	&90.2 	&91.2 	&75.0 	 	&88.0 &74.1 	&83.0   \\
        ~& - w/ RRR + Lemma  &40k  & 85.0          & 85.4 & \textbf{84.1} & 90.4& \textbf{92.5}  & 74.7  &  \textbf{88.2}  &  74.7 & 83.1 \\
        

        
        
        \bottomrule
    \end{tabular}
    }
    \caption{Full scores of ablation on AMRization methods.}

    \label{tab:amrization}
\end{table*}


==> table/amrization.tex <==
% \begin{table*}[t]
%     \centering
%     \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{llccccccccccc}
%         \toprule
%                 ~& \multirow{2}{*}{Model} &\multirow{2}{*}{Extra Data} & \multirow{2}{*}{\textsc{smatch}} &
%                 \multirow{2}{*}{NoWSD} &
%                 \multicolumn{4}{c}{Concept-related} & \multicolumn{3}{c}{Topology-related} \\
%                 \cmidrule(r){6-9} \cmidrule(r){10-12} 
%         ~ & ~ & ~ & ~& ~ & Conc. & NER & Neg. & Wiki. & Unll. & Reen. & SRL \\
%         \midrule
        

%         \multirow{8}{*}{\rotatebox[origin=c]{90}{{AMR 2.0}}}      

%         ~& \textbf{Ours (w/ Semantic Role Labeling) } &40k &84.5 &84.9 &90.2 & 91.8&74.6&84.0&87.7 &74.2 &82.8 \\
%         ~& - w/ Arg. Reduction(AR) &40k &84.8 &85.2 &90.4 &92.2 &74.2&83.9&88.1 & 74.5 &83.0  \\
%         ~& - w/ Reen. Restoration(RR)  &40k &85.0 &85.4&90.6 & 92.1 &75.6&83.5&\textbf{88.2}&\textbf{75.5}&\textbf{83.7}\\
%         ~& - w/ AR+RR  &40k    &\textbf{85.1}   &\textbf{85.6}  &90.4  & 91.4  & \textbf{75.7} &  83.6 & \textbf{88.2} & 75.0  &  83.5   \\
       
%         ~& \textbf{Ours (w/ Dependency Parsing) } &39k  &84.4 &84.9 &90.1&90.5 &73.5 & 82.9&87.8 &74.3 &82.9 \\
%         ~& - w/ Redundant Relation Removal (RRR) &39k & 84.5 & 	85.0	&90.2 	&91.2 	&74.3 	&83.5 	&88.0 &74.5 	&82.9  \\
%         ~& - w/ Lemmatization (Lemma)  &39k & 84.7 	& 	85.2 	&90.2 	&91.2 	&75.0 	&83.8 	&88.0 &74.1 	&83.0   \\
%         ~& - w/ RRR + Lemma  &39k  & 85.0          & 85.4 & 90.4& \textbf{92.5}  & 74.7 &  84.1  &  \textbf{88.2}  &  74.7 & 83.1 \\
        
%         % \cmidrule{2-12}
%         % ~& \citet{bevil-spring} (Ensemble)       &N     & 84.2  &  \\
%         % ~& - w/ AR+RR (Ensemble) &40k  &\textbf{85.3}            & \textbf{85.7} & 90.7 & 92.2  & 75.0 &  83.9  &  \textbf{88.4}  & \textbf{75.0} & \textbf{83.6}   \\
%         % ~&  - w/ RRR + Lemma (Ensemble) &39k  & 85.1        & 85.6 & \textbf{90.8} & \textbf{92.8}  & \textbf{77.7} &  \textbf{84.1}  &  \textbf{88.4}  &  \textbf{75.0} & 83.3 \\
        
        
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Analysis on AMRization methods}

%     \label{tab:amrization}
% \end{table*}


\begin{table}[t]
    \centering
    \resizebox{0.4\textwidth}{!}{
\begin{tabular}{lccc}
        \toprule
             Model & \textsc{Smatch} & Conc. & Topo. \\
        \midrule
         \textbf{Ours (w/ Semantic Role Labeling) } &84.5  & 85.5  & 81.6 \\
         - w/ Arg. Reduction(AR)   &  84.8  & 85.6  & 81.9\\
         - w/ Reen. Restoration(RR)   & 85.0  & 86.1  & \textbf{82.5} \\
         - w/ AR+RR &  85.1  & 85.8  & 82.2 \\ 
         - w/ AR+RR$^D$  &\textbf{85.2}  & \textbf{86.2}  & 82.1 \\ 
        \midrule
         \textbf{Ours (w/ Dependency Parsing) } & 84.4  & 84.7  & 81.7  \\
          - w/ Redundant Relation Removal (RRR)   &84.5  & 85.2  & 81.8   \\    
         - w/ Lemmatization (Lemma)     & 84.7  & 85.5  & 81.7\\    
         - w/ RRR + Lemma &\textbf{85.0}  & \textbf{85.9}  & \textbf{82.0}\\
        \bottomrule
    \end{tabular}}
    \caption{We report the average scores of Concept-related scores and Topology-related scores. The full scores are listed in Table~\ref{tab:amrization}. The improvement of involving all techniques against trivial linearization is significant with p < 0.005 for both SRL and DP.}
    \label{tab:amrization_small}
\end{table}








==> table/dataset.tex <==
\begin{table}[h]
\centering
\scalebox{0.95}{
\begin{tabular}{ccccc}
        \toprule
         Dataset &Task & Train & Validation \\
        \midrule
        CNNDM & Summarization & 40k & 1k \\
        DialogSum & Summarization & 13k & 0.5k \\
        EN-DE & Translation & 40k & 3k \\
        DE-EN & Translation & 40k & 3k \\
        Ontonotes & SRL & 40k & 1.5k \\
        PTB3 & DP & 39k & 1.7k \\

        \bottomrule
    \end{tabular}}
    \caption{Dataset introduction}

    \label{tab:dataset}
\end{table}

==> table/dp_amrizatiton.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{1\textwidth}{!}{%
\begin{tabular}{llccccccccccc}
        \toprule
                ~& \multirow{2}{*}{Model} &\multirow{2}{*}{Extra Data} & \multirow{2}{*}{\textsc{smatch}} &
                \multirow{2}{*}{NoWSD} &
                \multicolumn{4}{c}{Concept-related} & \multicolumn{3}{c}{Topology-related} \\
                \cmidrule(r){6-9} \cmidrule(r){10-12} 
        ~ & ~ & ~ & ~& ~ & Conc. & NER & Neg. & Wiki. & Unll. & Reen. & SRL \\
        \midrule
        

        \multirow{7}{*}{\rotatebox[origin=c]{90}{{2.0}}}      
                                          
        ~& \citet{bevil-spring}       &N     & 83.8  & 84.4 & 90.2 & 90.6 & 74.4 & 84.3 & 86.1 & 70.8 & 79.6 \\
        ~& \citet{bevil-spring} (w/ silver)   &200k     & 84.3 & 84.8 & 90.8 & 90.5 & 73.6 & 83.1 &  86.7 &  72.4 & 80.5 \\
        ~& \textbf{Ours (w/ Dependency Parsing) } \\
        ~& - w/ Trivial Linearization &39k  \\
        ~& - w/ Redundant Relation Removal (RRR) &39k &     \\
        ~& - w/ Lemmalization (Lemma)  &39k & 84.7 	& 	85.2 	&90.2 	&91.2 	&75.0 	&83.8 	&88.0 &74.1 	&83.0   \\
        ~& - w/ RRR + Lemma  &39k  & \textbf{85.0}            & \textbf{85.4} & \textbf{90.4} & \textbf{92.5}  & \textbf{74.7} &  84.1  &  \textbf{88.2}  &  \textbf{74.7} & \textbf{83.1} \\
        \bottomrule
    \end{tabular}
    }\caption{Analysis on DP's AMRization methods}

    \label{tab:srl_amr}
\end{table*}



==> table/effect_r2l.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.3\textwidth}{!}{
\begin{tabular}{lcc}
        \toprule
             Model & \textsc{Smatch} \\
        \midrule
             AMRBART (Ours) & 85.3 \\
             RGL \textbf{w/ R2L} (Ours) & 86.1 \\
             RGL \textbf{w/ L2R} (Ours) & 85.8 \\

        \bottomrule
    \end{tabular}}
    \caption{Effect of the different linearization orders to the model. "RGL \textbf{w/ R2L}" is the RGL model where we feed the reverse graph linearization as the extra input. "RGL \textbf{w/ L2R}" is the control group where we feed the standard L2R linearization to the graph encoder of the model without changing other conditions. }
    \label{tab:effect_r2l}
\end{table}


==> table/fewshot.tex <==
 \begin{table}[t]
    \centering
\scalebox{0.8}{
\begin{tabular}{lllccc}
        \toprule
          ~&Model&BOLT  & LORELEI & DFA \\
        \midrule
        \multirow{2}{*}{\rotatebox[origin=c]{0}{Dev}}
         ~ &SPRING & 30.8  & 72.3 & 73.5\\
         ~ &\textbf{Ours} &\textbf{56.0}  & \textbf{73.9} & \textbf{76.1}\\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{0}{Test}}
         ~&SPRING &34.6  &73.8 & 71.1\\
         ~&\textbf{Ours} &\textbf{59.4}  & \textbf{74.5} &\textbf{74.3}\\
        \bottomrule
    \end{tabular}}
    \caption{Model Smatch scores in the low-resource setting. There are 1061, 4441, 6455 examples in the training set of BOLT, LORELEI and DFA, respectively. The model exploits SRL as the intermediate task.}

    \label{tab:few}
\end{table}

==> table/finetuning_select.tex <==
\begin{table}[t]
    \centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{lccc}
        \toprule
          Model&Extra & \textsc{Smatch} \\
        \midrule
         
         \textbf{Ours (w/ Intermediate) } \\
         - w/ DP & 40k & 85.0 \\    
         - w/ SRL &   40k  &\textbf{85.1}     \\  
         - w/ DP,SRL & 80k & 84.7 \\  
         \textbf{Ours (w/ Multitask) } \\
         - w/ DP &40k & 83.7 \\
         - w/ SRL &40k &  83.6   \\
         - w/ DP,SRL &80k & 83.5   \\
         \textbf{Ours (w/ Multi. + Inter.) } \\
         - w/ DP &40k &84.1  \\
         - w/ SRL &40k & 84.1    \\
         - w/ DP,SRL &80k & 83.9    \\
        
        \bottomrule
    \end{tabular}}
    \caption{Analysis on Training Paradigms. Intermediate-task training is more suitable for AMR parsing than Multitask training}

    \label{tab:funetuning}
\end{table}

==> table/task_select.tex <==


\begin{table*}[htb]
    \centering
    \resizebox{1\textwidth}{!}{%
\begin{tabular}{llccccccccccc}
        \toprule
                ~& \multirow{2}{*}{Model} &\multirow{2}{*}{Extra Data} & \multirow{2}{*}{\textsc{smatch}} &
                \multirow{2}{*}{NoWSD} &
                \multicolumn{4}{c}{Concept-related} & \multicolumn{3}{c}{Topology-related} \\
                \cmidrule(r){6-9} \cmidrule(r){10-12} 
        ~ & ~ & ~ & ~& ~ & Conc. & NER & Neg. & Wiki. & Unll. & Reen. & SRL \\
        \midrule
        

        \multirow{7}{*}{\rotatebox[origin=c]{90}{{2.0}}}      
                                          
        ~& \citet{bevil-spring}       &N     & 83.8  & 84.4 & 90.2 & 90.6 & 74.4 & \textbf{84.3} & 86.1 & 70.8 & 79.6 \\
        ~& \citet{bevil-spring} (w/ silver)   &200k     & 84.3 & 84.8 & \textbf{90.8} & 90.5 & 73.6 & 83.1 &  86.7 &  72.4 & 80.5 \\
        ~& \textbf{Ours (w/ NLG Task) } \\
        ~& - w/ DialogSum & 13k & 84.5 &84.9 & 90.2&91.5 &74.8 &82.0 &87.8 &74.1 & 82.7 \\
        ~& - w/ CNNDM   & 40k & 84.4 &84.9 & 90.1& 91.5&74.8 &82.7 &87.7 & 74.6& 82.8 \\
        ~& - w/ DE-EN   & 40k &84.4 &84.9 &89.9&90.8&73.3&83.1&87.6&74.1&82.8\\ 
        ~& - w/ EN-DE   & 40k &84.0 &84.3 &89.7 &90.9 &74.3 &83.2 &87.1 &73.5 &81.9\\ 
        ~& \textbf{Ours (w/ Parsing Task) } \\
        ~& - w/ DP & 39k & 85.0          & 85.4 & 90.4 & \textbf{92.5}  & 74.7 &  84.1  &  \textbf{88.2}  &  74.7 & 83.1 \\    
        ~& - w/ SRL &   40k  &\textbf{85.1}   &\textbf{85.6}  &90.4  & 91.4  & \textbf{75.7} &  83.6 & \textbf{88.2} & \textbf{75.0}  &  \textbf{83.5}       \\    
        \bottomrule
    \end{tabular}
    }
    \caption{Analysis on Task Selection}

    \label{tab:task_sel}
\end{table*}

==> table/task_small.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.45\textwidth}{!}{
\begin{tabular}{lccccc}
        \toprule
             Model &Extra & \textsc{Smatch} & Conc. & Topo.  \\
        \midrule
         \textbf{Ours (w/ NLG) } \\
         - w/ DialogSum & 13k & 84.5 &85.5 &81.5\\
         - w/ CNNDM   & 40k & 84.4 &85.5 &81.7 \\
         - w/ CNNDM   & 80k & 84.2 &85.1 &81.4 \\
         - w/ EN-DE   & 40k &84.4 &85.3&81.5 \\ 
         - w/ EN-DE   & 80k &84.4& 85.4 &81.4 \\ 
         - w/ EN-DE   & 200k&84.2&84.6 &81.2 \\ 
         - w/ EN-DE   & 400k &83.6 &84.9 & 80.6  \\
         \textbf{Ours (w/ Parsing) } \\
         - w/ DP & 40k & 85.0&\textbf{85.9}&   82.0 &  \\    
         - w/ SRL & 40k  &\textbf{85.1} &85.8 &\textbf{82.2}   \\    
        \bottomrule
    \end{tabular}}
    \caption{Result of Task Selection. We first train BART on different auxiliary tasks for 10 epochs before AMR Parsing. We also report the average scores of Concept-related (Conc.) and Topology-related metrics (Topo.) }
    \label{tab:task_sel_small}
\end{table}

